Latitudinal Propagation of Thermal Rossby Waves in Stellar Convection Zones

Using an analytic model, we derive the eigenfrequencies for thermal Rossby waves that are trapped radially and latitudinally in an isentropically stratified atmosphere. We ignore the star's curvature and work in an equatorial f-plane geometry. The propagation of inertial waves is found to be sensitive to the relative direction of the wave vector to the zonal direction. Prograde propagating thermal Rossby waves are naturally trapped in the radial direction for frequencies above a critical threshold, which depends on the angle of propagation. Below the threshold frequency, there exists a continuous spectrum of prograde and retrograde inertial waves that are untrapped in an isentropic atmosphere, but can be trapped by gradients in the specific entropy density such as occurs in a stellar convection zone. Finally, we discuss the implications of these waves on recent observations of inertial oscillations in the Sun, as well as in numerical simulations.

==> Reviewer_Report.tex <==
The changes are marked in Magenta in the manuscript.
Reviewer:
This paper extends analysis of thermal Rossby waves in the solar convection zone, focusing specifically on latitudinal propagation and trapping. Trapping is particularly important as guidance to helioseismologists for what latitudes to focus on to see these waves. This paper represents a useful addition to the growing literature on solar Rossby waves. I have some modest, but hopefully helpful, suggestions for improvement, before final acceptance.

Reply: We thank the reviewer.

1. The title seems a little narrow. The analysis applies to stellar convection zones generally. Instead of 'in the solar convection zone', why not say 'in solar and stellar convection zones'. This suggestion is made in part because there is a possibility that thermal Rossby waves of the type being analyzed may not be a significant component of solar Rossby waves, since solar rotation may be too slow, but surely there are other stars with substantial convection zones that are rotating fast enough that thermal Rossby waves should be important. Some recognition of this possibility for the Sun would be appropriate, since thermal Rossby waves have yet to be observed in the solar case. See also item 4 below, which suggests even broader applicability.

Reply: Sure. We have changed the title to "Latitudinal Propagation of Thermal Rossby Waves in Stellar Convection Zones" and added a couple of sentences in the "Introduction" section.

2. Some additional discussion of the range of solar Rossby waves that are observed so far would be appropriate. Even though the solar convection zone is both deep and contains a large density decline with radius, nevertheless Rossby waves of the 'classical' Rossby-Haurwitz type, the favored modes for thin stably stratified spherical shells, are observed. This says that thin shells are sufficient for such classical waves, but apparently not necessary. What do the authors make of this puzzle?

Reply: This is a very good idea and the work is already being carried out and so we prefer to defer it for a later paper.

3. The mathematics is well laid out and carefully done. Limiting the analysis to an equatorial channel or annulus has significant mathematical advantages, fully appropriate at this stage of the analysis. While certain prior work on solar inertial oscillations is cited, the authors can make direct comparison with prior results found in Gilman 1987 (ApJ, 318, 904). Despite the purpose there was highlighting the roles of inertial oscillations in solar differential rotation, some comments on how their thermal Rossby waves might be affected by radial differential rotation would be helpful. If it is possible to add a radial rotation gradient to the analysis, it could give interesting results, for either this or a later paper.

Reply: This is an important issue, but in the current paper we wish to avoid a detailed discussion of the critical layers that become possible with nonuniform rotation.  Therefore, we have included a brief motivation for why we have adopted uniform rotation. This is done in the first paragraph of the Model section.

5. Solar and stellar Rossby waves are seldom studied in equatorial channels, with or without explicit cylindrical geometry, but such a configuration is common in studying Rossby waves and instabilities in accretion disks. In fact there is a substantial literature on this topic -- see, e.g., Lin, M.K. ApJ,754,21(2012). Stratification and density gradients perpendicular to the rotation axis play a role. It would be good to make connections with that literature and results.

Reply: We have added "While there is a rich literature on Rossby waves in stratified astrophysical disks \citep[e.g.,][]{Li2000, Lin2012}, to date only a few studies have explored how thermal Rossby waves propagate through a stratified star \citep{Glatzmaier1981, Gilman1987, Hindman2022, Hindman2023}" in the last paragraph of the Introduction section.

6. To make better comparison with the spherical problem, some discussion on relating their cartesian wavenumber k_x to the spherical shell longitude wave number 'm' can help the readers to get a better idea of the physical scale of the modes being discussed. Latitude is much harder, but some statement about latitude extent is appropriate.

Reply: This was already mentioned in Figure 5 and we have now explicitly mentioned it in Figure 3 for spherical harmonic degree as well.
